High Performance Evaluation of Helmholtz Potentials using the Multi-Level Fast Multipole Algorithm

Evaluation of pair potentials is critical in a number of areas of physics. The classicalN-body problem has its root in evaluating the Laplace potential, and has spawned tree-algorithms, the fast multipole method (FMM), as well as kernel independent approaches. Over the years, FMM for Laplace potential has had a profound impact on a number of disciplines as it has been possible to develop highly scalable parallel algorithm for these potential evaluators. This is in stark contrast to parallel algorithms for the Helmholtz (oscillatory) potentials. The principal bottleneck to scalable parallelism are operations necessary to traverse up, across and down the tree, affecting both computation and communication. In this paper, we describe techniques to overcome bottlenecks and achieve high performance evaluation of the Helmholtz potential for a wide spectrum of geometries. We demonstrate that the resulting implementation has a load balancing effect that significantly reduces the time-to-solution and enhances the scale of problems that can be treated using full wave physics.

==> Introduction/Introduction0.1.tex <==
Physics described by hyperbolic partial differential equations (PDEs) forms the backbone of a wide array of modern technologies. Solutions to PDEs governing electromagnetics and acoustics have enabled technologies that have had, and will continue to have, a broad and profound effect on our daily lives. The common thread for the wide range of phenomena described by the Helmholtz equation is understanding and manipulation of wave physics at multiple length scales. This task is increasingly challenging given the increase in geometric complexity (smaller and more complex features) and wider range of operating frequencies (requiring more precision and detail to achieve optimal performance at all frequency bands). Advances in these technologies, and engineering sophisticated yet robust systems, are intimately tied to a detailed understanding of the underlying wave physics. Today, more often than not, such insight requires simulations via high-fidelity computational tools.

One of the main challenges in developing such tools is computing fields on electrically large objects, where the electrical length is measured in terms of the largest linear dimension in wavelengths. For several emerging problems, the electrical length is several thousand wavelengths. Creating a full-wave physics based model for such ``large'' Helmholtz systems represents a major challenge because at its core, a Helmholtz solver requires the solution of an $N$-body problem. Means to alleviate the $\mathcal{O}(N_{s}^2)$ cost of the direct evaluation scheme, where $N_{s}$ is the number of sources (or degrees of freedom) in the discretization, follows from the basic observation that interaction potentials can be represented with controllable accuracy by using an addition theorem; for non-oscillatory potentials a Taylor series provides one means of deriving such an addition theorem. This insight gave rise to tree algorithms, the most famous of which is FMM\,\cite{Greengard1987}. By exploiting this alternate representation, in FMM interactions among sufficiently far away source-observer pairs are reduced to computationally inexpensive approximations. The resulting hierarchical algorithm has an asymptotically linear cost of $\mathcal{O}(N_s)$ and enables the solution of $N$-body problems that are otherwise impractical.

\paragraph{Laplace vs. Helmholtz FMM} FMM for the Laplace equation (L-FMM) has been explored in depth, to a large extent driven by gravitational physics \cite{Warren1993} and electrostatic interactions. In contrast, advances for Helmholtz FMM (H-FMM) have been limited because challenges in solving the Helmholtz equation are significantly different than those of the Laplace equation. Potentials associated with the Laplace equation are non-oscillatory and inversely proportional to the distance between two points. As a result, the number of multipoles chosen needs only to accurately reconstruct the \textit{magnitude}, and is fixed for any node in a tree. In stark contrast, for Helmholtz systems, the number of multipoles {\em must} be chosen so as to accurately represent \textit{both phase and magnitude}. Therefore, \emph{the information content in an H-FMM node is proportional to the square of the node's electrical/acoustic size, and quadruples at each level of the H-FMM tree}.

This fundamental difference leads to major scalability and memory bottlenecks in H-FMM implementations. In particular, as one ascends an octree ($l\rightarrow l+1$), at each level the number of nodes decreases by (roughly) a factor of {\em four} for surface geometries, and {\em eight} for volumetric systems. Due to the constant information content in L-FMM nodes, the per-level cost of far-field interactions falls off exponentially, and the bulk (80-90\%) of the work in L-FMM is found at the leaves. Thus, existing L-FMM efforts have focused on optimizing the computation and masking communication costs primarily at the leaf level\,\cite{ying2004kernel,sundar2008bottom,agullo2014task}. On the other hand, due to the quadrupling of the information content as one ascends an H-FMM tree, the computational and memory costs in H-FMM stay constant for each tree level for surface geometries (which constitutes the majority of H-FMM application problems) and decays slowly for volumetric problems. While a variant of the Laplace FMM algorithm called the multilevel fast multipole algorithm (MLFMA) \cite{song1997multilevel} has been developed for Helmholtz problems, advances in L-FMM do not translate readily to H-FMM. As such, the performance and scaling of MLFMA implementations have been limited.

\paragraph{Contribution}  
%The objective of this work is to develop an efficient parallel MLFMA implementation with controllable accuracies for electrically large domains that comprise non-uniform discretizations. While it is known that a particular class of tree traversal operators can ensure controllable accuracy \cite{Melapudi2011,Sarvas2003}, their use brings a set of challenges, especially for deep H-FMM trees. As elucidated in Sect.\,\ref{sec:algo_base}, the critical bottlenecks that arise are (a) memory requirements, and (b) load balancing deep non-uniform H-FMM trees. In this paper, we utilize a hybrid tree traversal scheme (see Section\,\ref{sec:hybrid}) which significantly reduces the overall memory requirements and we present an efficient parallelization of this hybrid scheme. Then in Section\,\ref{sec:loadbalancing}, we present an empirical load balancing tehcnique to ensure scalable computations with electrically large objects. As shown through extensive numerical tests in Sect.\,\ref{sec:performance}, our proposed techniques achieve significant speedup over existing approaches, all with controllable accuracy.
The objective of this work is to demonstrate a method of improving the parallel execution of the high levels of the tree, where the number of nodes is less than the number of processes, making course grain parallelization impractical by:

\begin{enumerate}
  \item Provide an algorithm with fine grain parallelization at higher levels of the tree where the number of processes exceed the number of nodes.
  \item Provide a detailed analytical model of the complexity and memory use of the entire tree traversal algorithm with the added fine grain parallelization.
  \item Demonstrate the accuracy of the analytical model, and scalability of the overall algorithm, in a number of test scenarios.
\end{enumerate}


==> tikz3D.tex <==
\usetikzlibrary{calc,fadings,decorations.pathreplacing}
%% helper macros

\newcommand\pgfmathsinandcos[3]{%
  \pgfmathsetmacro#1{sin(#3)}%
  \pgfmathsetmacro#2{cos(#3)}%
}
\newcommand\LongitudePlane[3][current plane]{%
  \pgfmathsinandcos\sinEl\cosEl{#2} % elevation
  \pgfmathsinandcos\sint\cost{#3} % azimuth
  \tikzset{#1/.estyle={cm={\cost,\sint*\sinEl,0,\cosEl,(0,0)}}}
}
\newcommand\LatitudePlane[3][current plane]{%
  \pgfmathsinandcos\sinEl\cosEl{#2} % elevation
  \pgfmathsinandcos\sint\cost{#3} % latitude
  \pgfmathsetmacro\yshift{\cosEl*\sint}
  \tikzset{#1/.estyle={cm={\cost,0,0,\cost*\sinEl,(0,\yshift)}}} %
}
\newcommand\DrawLongitudeCircle[2][1]{
  \LongitudePlane{\angEl}{#2}
  \tikzset{current plane/.prefix style={scale=#1}}
   % angle of "visibility"
  \pgfmathsetmacro\angVis{atan(sin(#2)*cos(\angEl)/sin(\angEl))} %
  \draw[current plane] (\angVis:1) arc (\angVis:\angVis+180:1);
  \draw[current plane,dashed] (\angVis-180:1) arc (\angVis-180:\angVis:1);
}
\newcommand\DrawLatitudeCircle[2][1]{
  \LatitudePlane{\angEl}{#2}
  \tikzset{current plane/.prefix style={scale=#1}}
  \pgfmathsetmacro\sinVis{sin(#2)/cos(#2)*sin(\angEl)/cos(\angEl)}
  % angle of "visibility"
  \pgfmathsetmacro\angVis{asin(min(1,max(\sinVis,-1)))}
  \draw[current plane] (\angVis:1) arc (\angVis:-\angVis-180:1);
  \draw[current plane,dashed] (180-\angVis:1) arc (180-\angVis:\angVis:1);
}

%% document-wide tikz options and styles

\tikzset{%
  >=latex, % option for nice arrows
  inner sep=0pt,%
  outer sep=2pt,%
  mark coordinate/.style={inner sep=0pt,outer sep=0pt,minimum size=3pt,
    fill=white,circle}%
}
